Probabilistic Visual Place Recognition for Hierarchical Localization

Visual localization techniques often comprise a hierarchical localization pipeline, with a visual place recognition module used as a coarse localizer to initialize a pose refinement stage. While improving the pose refinement step has been the focus of much recent research, most work on the coarse localization stage has focused on improvements like increased invariance to appearance change, without improving what can be loose error tolerances. In this letter, we propose two methods which adapt image retrieval techniques used for visual place recognition to the Bayesian state estimation formulation for localization. We demonstrate significant improvements to the localization accuracy of the coarse localization stage using our methods, whilst retaining state-of-the-art performance under severe appearance change. Using extensive experimentation on the Oxford RobotCar dataset, results show that our approach outperforms comparable state-of-the-art methods in terms of precision-recall performance for localizing image sequences. In addition, our proposed methods provides the flexibility to contextually scale localization latency in order to achieve these improvements. The improved initial localization estimate opens up the possibility of both improved overall localization performance and modified pose refinement techniques that leverage this improved spatial prior.

==> tex/archived.tex <==

Visual Place Recognition (VPR) systems are used to localize a robot within an existing map consisting of a set of \textit{reference images} using one or more \textit{query images}. The query and reference images are typically temporally aligned, corresponding to frames subsampled from a video feed captured by the robot during map building and localization. A typical localization pipeline for single image VPR is in essence an image retrieval problem. It involves comparing a query image against each reference image and attributing to each image comparison a \textit{quality score}. Quality scores are subsequently filtered out to reject potential false matches, and the highest scoring match that remains is a \textit{localization proposal} made by the model. The robot then inherits the pose corresponding to this retrieved reference image. 

One major innovation was to use image sequences in the retrieval process instead of single images and it has been shown that this yields much more discriminative matching performance when localizing between traverses captured with extreme appearance changes in between such as day vs. night. One disadvantage of these methods however, is in the requirement of matching fixed length sequences between query and reference images, which requires accumulating a potentially long sequence of query images before localizing. In contrast, we propose \textit{online algorithms} based on probabilistic filtering that process images incrementally and localizes as soon as a measure of confidence in the belief of the robot state is sufficiently high. In practice, we see that these algorithms tend to localize in less time steps for environments with lower levels of perceptual aliasing.

In addition, there has been much research effort at generating more effective low dimensional image representations for VPR which tend to cluster images in the feature-vector space that are captured close to each other in terms of pose despite appearance changes \cite{Arandjelovic16}, \cite{Torii15}, \cite{Sunderhauf15}. To that effect, we introduce our filtering algorithms agnostic to the exact visual front-end used and provide a heuristic for model parameter calibration to minimize parameter tuning when changing front-ends.

A key motivation for developing VPR systems is to localize a robot to a pre-built metric map built by existing visual SLAM systems. In fact, a number of visual SLAM (VSLAM) frameworks based on either direct image alignment \cite{Engel14} or indirect, feature-based methods \cite{MurArtal15} use a VPR system for loop closure and/or relocalization when tracking is lost. Similarly in the context of 6-DoF visual localization (VLoc) \cite{Sattler2018}, VPR is used as an initial filtering step to a more sophisticated geometric pose refinement method when localizing a camera within a point cloud map built offline by Structure-from-Motion (SfM) pipelines. A requirement of VPR methods in this context is the ability to localize accurately enough to either reliably initialize the optimizers present in a VSLAM back-end based on say direct image alignment or sufficiently reduce the search space within the point cloud for feature-based camera resectioning. This can be thought of as an initial \textit{coarse} localization step used to initialize a more accurate geometry-based optimization back-end to refine the true robot pose as discussed in \cite{Sarlin19}. From this, we can see that another requirement of VPR systems is to be scalable and fast to ensure localization scales favorably to map size, especially compared to brute forcing the pose refinement step (e.g. exhaustive 2D-3D matching to the entire point cloud in the VLoc context). We demonstrate our methods satisfy both of these requirements in our experiments.

Finally, a contribution of this paper is a particle filter localization algorithm that uses pose estimates of reference images and odometry readings in the query sequence. In the context of VLoc, reference images are used to build the point cloud and SfM pipelines typically estimate the poses of all images simultaneously with the position of the 3D points in the point cloud. Similarly, many state-of-the-art VSLAM systems are keyframe-based systems, and pose estimates for these keyframes are estimated and refined in the mapping stage. In addition, robots are typically equipped with ego-motion sensors which can be used to yield odometry measurements between images in the query sequence, for example inertial measurement units (IMUs), visual odometry (VO).

The rest of this paper is structured as follows. First, we will review the literature and discuss similar work. Then, we will introduce the methodology of our localization algorithms. Finally, we will assess performance of our method against other existing methods and baselines.


\subsubsection{Bootstrap Filter with Adaptive Resampling}\label{ssec:bootstrap}

This is the basic formulation of our localization algorithm and is the particle filter formulation used in \cite{Dellaert-1999}. Assuming we have a set of particles $\cX_t$ representing the marginal posterior at time step $t$, the standard bootstrap filter updates each particle by drawing a sample from the motion prior distribution and updating the particle weights proportional to the likelihood of observing the image descriptor given the particle's new location. In addition, we implement a form of \textit{adaptive resampling}, where particles are resampled at various time steps proportional to the particle weights to mitigate sample impoverishment \cite{doucet2009tutorial}, which is the case where a very small number of particles have all of the weight. Resampling is performed according to the Effective Sample Size (ESS) heuristic, specifically when the ESS of the particles reaches below a certain level. The high-level pseudocode of this method is summarized in Algorithm \ref{alg:bootstrapfilter}.

\begin{algorithm}\label{alg:bootstrapfilter}
\caption{Bootstrap filter localization}
\SetAlgoLined
\KwResult{Robot pose $\widehat{\bT}\in\SE$ or localization failure.}
 Set $t=1$\;
 Initialize $\cX_1$ with $M$ samples from $\mu(\bT_1 | \bz_1, \cM)$\;
 \While{$t < t_{max}$}{
  $t=t+1$\;
  \tcp{Update particle poses and weights}
  \For{$i=1,\dots,M$} 
    {
        $\bTi{i}_{t} \sim f(\bT_t  |\bTi{i}_{t-1}, \bU_{t-1})$\;
        $\wi{i}_{t} \propto \wi{i}_{t-1} \cdot g(\bz_{t} | \bTi{i}_{t}, \cM)$\;
    }
  Normalize weights\;
  $\cX_{t} = \{(\wi{i}_{t}, \bTi{i}_{t})\}_{i=1}^M$ \;
  \tcp{Predict pose if particles converged}
  $\tau_t=\convergencecriterion(\cX_t)$\;
  \If{$\tau_t < \tau_{thres}$}
  {
  $\widehat{\bT} = \localize(\cX_t)$\;
  \textbf{break}\;
  }
  \tcp{Adaptive resampling (systematic)}
  \If{ESS $< pM$ for $p \in (0, 1)$}{
   $\widehat{\cX}_t = \emptyset$\;
   $u_1 \sim \cU\left[0, \frac{1}{M}\right]$\;
   $u_i = u_1 + \frac{i-1}{M}$ for $i\in\{2,\dots,M\}$\;
   \For{$i=1,\dots,M$}
   {
   \tcp{Note: define $\sum_{k=1}^{0}\coloneqq 0$}
   $i^* = \argmin_{j} \sum_{k=1}^{i-1} \wi{k}_t \leq u_j \leq \sum_{k=1}^{i}\wi{k}_t$\; 
   $\widehat{\cX}_t = \widehat{\cX}_t + \cX_t^{(i^*)}$
   }
   $\cX_t = \widehat{\cX}_t$\;
   }
 }
\end{algorithm}

We will discuss in detail the $\convergencecriterion$ and $\localize$ functions in Section $\ref{ssec:localization}$. In addition, note that while there are alternative particle resampling methods, the systematic resampling method we have chosen is both effective and easy to implement as suggested in \cite{doucet2009tutorial}.

Our experiments show that the bootstrap filter does not perform well in the localization task, even for large numbers of particles. To address this problem, we introduce a more advanced filtering algorithm called the \textit{auxiliary particle filter}.




Localization can be formulated as inferring some measure of central tendency using this marginal posterior distribution. Specifically, for each time $t$ we estimate the robot position $\widehat{\bT}_t$ using the posterior mean of the marginal distribution given by
\begin{align} 
    \widehat{\bT}_t = \bbE \left[ \bT_{t}  |\bz_{1:t}, \bU_{1:t-1}, \cM\right]. \label{eq:infermean}
\end{align}
Before delving into the specifics of the components of the state-space model $\mu$, $f$ and $g$, we discuss how we can use particle filtering methods in general to infer distributional quantities such as \eqref{eq:infermean} for a particular state-space model.


We can now specify a state-space model which characterizes the joint distribution over the image descriptors and unknown robot poses $\{\bT_1,...,\bT_T\}$ given the odometry readings and map to be
\begin{align}\label{eq:ssm}
    p(\bT_{1:T}, \bz_{1:T} | \bU_{1:T-1}, \cM) &= \nonumber\\
    \mu(\bT_1 | \bz_1, \cM)\prod_{t=2}^T g(\bz_t &| \bT_t, \cM)f(\bT_t | \bT_{t-1}, \bU_{t-1}),
\end{align}
where $f$ and $g$ are the \textit{motion prior} and \textit{observation} likelihood, respectively and $\mu$ is the \textit{initial prior} density relevant to particle initialization. These are analogous to the state transition density, observation likelihood and initial belief in the topological filter. Similarly to the discrete case, filtering algorithms such as particle filters or alternatively, variants on the Kalman filter can be used to efficiently estimate the marginal posterior at time $t$ given by $p(\bT_{t}  |\bz_{1:t}, \bU_{1:t-1}, \cM)$ instead of the higher-dimensional posterior distribution over the full robot trajectory $p(\bT_{1:t}|\bz_{1:t}, \bU_{1:t-1}, \cM))$. Much like HMMs, we can derive a recursive update for a state-space model using the relation 
\begin{align}\label{eq:analyticalupdate}
    p(\bT_{t+1}  |\bz_{1:t+1}, \bU_{1:t}, \cM) \propto &\nonumber\\
        g(\bz_{t+1} | \bT_t, \cM) &p(\bT_{t+1}  |\bz_{1:t}, \bU_{1:t}, \cM),
\end{align}
where the rightmost term in \eqref{eq:analyticalupdate} is given by
\begin{align}
    p(\bT_{t+1}  |\bz_{1:t}, \bU_{1:t}, \cM) = &\nonumber\\
    \int f(\bT_{t+1} | \bT_t, \bU_t) &p(\bT_{t}  |\bz_{1:t}, \bU_{1:t-1}, \cM) d\bT_t.
\end{align}
Particle filtering techniques typically provide methods for applying this update to a particle set such that the updated particles estimate the marginal posterior of the new time step. For more details on the theory behind particle filters, refer to \cite{doucet2009tutorial} and for a comprehensive treatment of probabilistic filtering approaches in robotics see \cite{Thrun2005}.



\subsubsection{Auxiliary Filter}\label{ssec:auxiliary}

The backbone of our particle filtering algorithm utilizes the auxiliary particle filter formulation. In contrast to the bootstrap filter found in the original MCL paper, the auxiliary filter performs the particle resampling step \textit{before} applying the motion update and image descriptor reweighting. In addition, this resampling step incorporates the image descriptor and odometry readings from the next time period and so the auxiliary filter is commonly referred to as a \textit{lookahead filter}. The weights used for the resampling step are computed from a set of arbitrary \textit{reference points}, which in our case are the points obtained after applying the raw odometry reading to the existing particle set. The pseudocode for the auxiliary filter algorithm is presented in Algorithm \ref{alg:auxiliaryfilter}. 

\begin{algorithm}\label{alg:auxiliaryfilter}
\caption{Auxiliary filter localization}
\SetAlgoLined
\KwResult{Robot pose $\widehat{\bT}\in\SE$ or localization failure.}
\textit{Localized = 0}\;
 Set $t=1$\;
 Initialize $\cX_1$ with $M$ samples from $\mu(\bT_1 | \bz_1, \cM)$\;
 \While{$t < t_{max}$}{
  $t=t+1$\;
  \For{$i=1,\dots,M$} 
    {
        $\bar{\bT}^{(i)}_t = \bTi{i}_{t-1} \cdot \bU_{t-1}$\text{\;} \tcp{reference point}
        $\bar{w}^{(i)}_{t} \propto \wi{i}_{t-1}  \cdot g(\bz_{t} | \bar{\bT}^{(i)}_t, \cM)$\text{\;} \tcp{aux weights}
    }
  Normalize auxiliary weights\;
  \tcp{Resample using aux weights}
  $\widehat{\cX}_t = \emptyset$\;
   $u_1 \sim \cU\left[0, \frac{1}{M}\right]$\;
   $u_i = u_1 + \frac{i-1}{M}$ for $i\in\{2,\dots,M\}$\;
   \For{$i=1,\dots,M$}
   {
   \tcp{Note: define $\sum_{k=1}^{0}\coloneqq 0$}
   $i^* = \argmin_{j} \sum_{k=1}^{i-1} \wi{k}_t \leq u_j \leq \sum_{k=1}^{i}\wi{k}_t$\; 
   $\widehat{\cX}_t = \widehat{\cX}_t + \cX_t^{(i^*)}$
   }
   $\cX_t = \widehat{\cX}_t$\;
  \tcp{Update resampled particles with motion}
  \For{$i=1,\dots,M$} 
    {
        $\bTi{i}_{t} \sim f(\bT_t  |\bTi{i}_{t-1}, \bU_{t-1})$\;
        $\wi{i}_{t} \propto \wi{i}_{t-1} \cdot \frac{g(\bz_{t} | \bTi{i}_{t}, \cM)}{g(\bz_{t} | \bar{\bT}^{(i)}_t, \cM)}$\;
    }
  $\cX_{t} = \{(\wi{i}_{t}, \bTi{i}_{t})\}_{i=1}^M$ \;
  \tcp{Predict pose if particles converged}
  Compute $\tau_t$ \eqref{eq:convergencecrit}\;
  \If{$\tau_t < \tau_{thres}$}
  {
  \textit{Localized = 1}\;
  Compute $\widehat{\bT}$ \eqref{eq:particleloc}\;
  \textbf{break}\;
  }
 }
  \If{Localized = 0}{
    Localization failure, restart filter\;
 }
\end{algorithm}

In practice, we observe that the auxiliary filter works better than the standard MCL formulation for a limited number of particles because updating particle positions using the motion prior when the motion prior has high variance tends to move some particles into regions where the posterior density is low and subsequently causes these particles to disappear in the resampling process. When this occurs to particles that are near the true robot pose, the final predicted robot pose will be incorrect. The auxiliary particle filter reduces the impact of this dramatically, since resampling occurs \textit{before} sampling from the motion prior and therefore increases the likelihood of having particles near the true robot pose. *show this using a figure of aux vs bootstrap* 

Now that we have introduced our particle filtering algorithms, we can now discuss how these particles are used for localization.


estimated posterior mean of the robot state given by
\begin{align} 
    \widehat{\bT}_t = \bbE \left[ \bT_{t}  |\bz_{1:t}, \bU_{1:t-1}, \cM\right]. \label{eq:infermean}
\end{align}
This is done by taking the sample mean over the particles
\begin{align}\label{eq:particleloc}
    \widehat{\bT}_t  &=  \begin{pmatrix}
                                        \bar{\bR} & \bar{\bt} \\
                                        \mathbf{0} & 1
                                        \end{pmatrix},
\end{align}
where $\bar{\bt}$ and $\bar{\bR}_t$ are estimates of the expected translation and rotation, respectively. For the mean rotation, we use the chordal distance formulation over $\SO$. Concretely,
\begin{align}
    \bar{\bt} = \sum_{i=1}^M \wi{i}_t\bti{i}_t, \quad \bar{\bR}_t = \argmin_{\bR} \sum_{i=1}^M\|\bR - \wi{i}_t \bRi{i}_t\|_F.
\end{align}
For more information on computing the expected rotation using rotation averaging, see \cite{hartley2013rotation}. Similar to the topological filter, we localize only when a confidence score computed from the particles is below a threshold $\tau_t <\tau_{thres}$. The confidence score for the particle filter is a measure of spatial uncertainty of the particles given by
\begin{align}\label{eq:convergencecrit}
    \tau_t = \sqrt{\max \left(\diag(\widehat{\bSigma}_t)\right)},
\end{align}
where $\diag(\widehat{\bSigma}_t)\in\bbR^6$ is the diagonal of the sample covariance matrix of the particles represented in the Lie algebra. Formally, let $\bxii{i}_t = \wi{i}_t\log \bTi{i}_t$ for all $i$, where $\log: \SE \rightarrow \se$ is the standard inverse exponential map. From this, we define $\widehat{\bSigma}_t$ as the sample covariance matrix for these weighted vector valued poses given by
\begin{align}
    \widehat{\bSigma}_t = \sum_{i=1}^M \left( \bxii{i}_t - \bar{\bxi}_t \right) \bW \left(\bxii{i}_t - \bar{\bxi}_t \right)^\top, \quad
   \bar{\bxi}_t = \sum_{i=1}^M \bxii{i}_t,
\end{align}
where $\bW$ is a diagonal weight matrix to rescale translation and attitude components. Intuitively, $\tau_t$ is the maximum standard deviation across any pose dimension.
